Fair Reinforcement Learning Algorithm for PV Active Control in LV Distribution Networks

The increasing adoption of distributed energy resources, particularly photovoltaic (PV) panels, has presented new and complex challenges for power network control. With the significant energy production from PV panels, voltage issues in the network have become a problem. Currently, PV smart inverters (SIs) are used to mitigate the voltage problems by controlling their active power generation and reactive power injection or absorption. However, reducing the active power output of PV panels can be perceived as unfair to some customers, discouraging future installations. To solve this issue, in this paper, a reinforcement learning technique is proposed to address voltage issues in a distribution network, while considering fairness in active power curtailment among customers. The feasibility of the proposed approach is explored through experiments, demonstrating its ability to effectively control voltage in a fair and efficient manner.

==> sections/IntroductionMauri.tex <==
% Context: The background of your topic
    %% current situation
The increase in the world energy consumption, the unstable cost of electricity and the goal of reducing the C02 emissions have led to a vast introduction of distributed energy resources (DER).\\
% Scope: The topic you’ll be covering
    %% introduction of DER (advantages)
These distributed devices are able to generate electricity from natural resources with low carbon emissions. Their main advantages, other than low emission electricity generation, is to reduce energy losses, since they are usually close to the consumption point, and helping decreasing the stress on the grids, especially during high-peak demand.
    %% what problem they cause (disavantages)
This more decentralised approach, however, increases the complexity of the grids. One of the possible consequences of DER devices is the opposite power flow when the energy produced exceeds the energy consumed. This opposite power flow increases the stress on the network, causing over-voltages and overloading of lines and nodes, power quality issues and other technical issues [\textcolor{red}{maybe cite papers}].\\
% Importance: Why your research matters in the context of an industry or the world
For this reason, the number of DER devices added into a grid has to be controlled by the distribution system operator (DSO). 
% from: State-of-the-art of hosting capacity in modern power systems with distributed generation
The total amount of DERs that can be added to a network, above which the system performances become unacceptable, is known as hosting capacity (HC).\\

%LR
As the interest has grown, many papers deal with HC evaluation [\textcolor{red}{cite papers with some focus on this implementation}]

%Paper goal
This paper intends to investigate ...

%Paper strucuture
The rest of the paper is organised as follows:

==> sections/LiteratureReview.tex <==
% Several studies on the field were already conducted. The authors in \cite{lr_frnn} predict the over-voltage instabilities using a recurrent neural network in a low-voltage distribution network. The authors forecast buses critical situations considering the voltage's phase angles information of consecutive buses instead of the voltage magnitudes; the tests are limited to a small network and time series are not taken in consideration. Thanks to its increasing popularity in many fields, some solutions for solving voltage problems have been proposed with reinforcement learning algorithms. The authors in \cite{gym-anm} developed environment playgrounds where they tested proximal policy optimisation and soft actor-critic algorithms. In \cite{lr_csi} a deep deterministic policy gradient algorithm is used to change active and reactive power of the generators.  
% \cite{lr_cmadarl} and \cite{lr_cfiq} control static VAR compensators and batteries to balance the voltage magnitude in a network, using multi deep reinforcement learning framework and control generators' reactive power respectively.\\
% %\cite{lr_cmadarl} used multi deep reinforcement learning framework to control static var compensators and batteries to balance the voltage magnitude in a network; for a similar task, the same authors, in \cite{lr_cfiq} control generators' reactive power. \\
% %in \cite{lr_fremi} authors control batteries and heat pumps to maximise energy consumption and reduce losses.\\

% The above-mentioned studies either: \emph{a)} consider only small test networks, \emph{b)} do not deal with unbalanced datasets, or \emph{c)} have high values of active curtailment. These are limitations since: \emph{a)} small networks may result in a not realistic analysis, \emph{b)} power grids are highly secure, thus the number of voltage problems is small with respect to the number of non-critical situations, \emph{c)} as the goal is to minimise losses, the generators' active power curtailment should be reduced to low values or avoided.\\
%%% ˆˆˆˆˆ OLD ˆˆˆˆˆ %%%

%%% NEW %%%
\textcolor{red}{OLTC}
Voltage control is a fundamental issue in power systems, and it has received significant attention in the literature. Historically, on-load tap changer (OLTC) technology has been utilized to regulate voltage output by adjusting the turns ratio of the transformer. This method has proven to be effective for voltage control in many applications.\\
However, as distributed energy resources (DERs) become increasingly prevalent in power systems, voltage violations can occur due to the variability and unpredictability of these resources. In such cases, OLTC may not be suitable due to the maintenance required after a limited number of tap changes to ensure its functionality.
% \textcolor{red}{cite papers?}
\\
Another technique used for voltage control is the Volt-VAr control. This technique involves the adjustment of devices' reactive power output to regulate the voltage, for example voltage regulators and capacitor banks. The primary advantage of this control is its ability to respond quickly to changes in load conditions and maintain voltage stability. However, the implementation of Volt-VAr control requires accurate measurements of voltage and reactive power, which can be challenging in some situations.\\

(Markushevich et. al., 2009) address the requirements for utilizing Voltage and Var Control for demand response, in an operating environment which includes Smart-Grid, Distribution Management Systems, Advanced Metering Infrastructure, Demand Response, and Distributed Energy Resources. The performance of voltage-source converter-based shunt and series compensators used for load voltage control in electrical power distribution systems has been analyzed and compared, when a nonlinear load is connected across the load bus (Gupta et. al., 2011). A methodology for voltage control in proposed by using the tap changing transformers and the inverters interfaced with the distributed generators (Oshiro et. al., 2011). Application of controllable customer equipment, Heat Pump Water Heater (HPWH), has been proposed in order to mitigate voltage violation (Mufaris et. al., 2013). (Ranamuka et. al., 2014) propose an online voltage control strategy for a realistic distribution system containing a synchronous machine-based renewable DG unit and other voltage regulating devices. An alternate method using an energy storage device to regulate the target PV bus voltage during ramp up/down of PV power is proposed (Chamana et. al., 2014). To that effect (Petinrin et. al., 2016) review the impact of renewable generations such as solar photovoltaic (PV) and wind energy on distribution system with voltage control strategies. The purpose of (Campaner et. al., 2016) is to show a possible undesired dynamic coupling of different reactive power control loops of network generators. In the paper, the interactions among DG units and voltage regulating devices are identified using their simultaneous and nonsimultaneous responses through time-domain simulations. For this task, an analytical technique is proposed and small signal modeling studies have been conducted (Ranamuka et. al., 2017). An optimal control strategy is proposed for minimizing VD and VF in PV-rich distribution systems (Mahmoud et. al., 2020).
